Interpretational errors in statistical causal inference

We formalize an interpretational error that is common in statistical causal inference, termed identity slippage. This formalism is used to describe historically-recognized fallacies, and analyse a fast-growing literature in statistics and applied fields. We conducted a systematic review of natural language claims in the literature on stochastic mediation parameters, and documented extensive evidence of identity slippage in applications. This framework for error detection is applicable whenever policy decisions depend on the accurate interpretation of statistical results, which is nearly always the case. Therefore, broad awareness of identity slippage will aid statisticians in the successful translation of data into public good.

==> Tables/Stochastic_LMTP_table.tex <==
\newgeometry{margin=1cm} 
\begin{landscape}
\thispagestyle{empty}
\newpage


%put your table here
{\renewcommand{\arraystretch}{1}
\begin{table}
\hspace*{-2cm}
\begin{threeparttable}

\caption{Additional stochastic mediation parameters \label{tab: altstoch}}

\vspace*{-2cm}

\begin{tabular}{|p{5cm}|p{2cm}|p{2cm}|p{7cm}|p{7cm}|}
\toprule
\multirow{2}{*}{\textbf{\emph{Parameter}} }& \multirow{2}{*}{\textbf{\emph{Author}}} & \multirow{2}{*}{\textbf{\emph{Name}}} &  \multicolumn{2}{|c|}{\textbf{\emph{Excerpts}}} \\ \cline{4-5} 
   & & &\multicolumn{1}{|c|}{\textbf{\textit{Identifiability}}} & \multicolumn{1}{|c|}{\textit{\textbf{Interpretability}} }     \\  \hline
   \\  \cline{2-2}\cline{4-5}  
 & & &  &   \\ \hline  \hline 
  \\ \hline  \hline 
\bottomrule
 \hline
\end{tabular}
 \begin{tablenotes}
      \tiny
      \item 
    \end{tablenotes}
\end{threeparttable}

\end{table}
}

\end{landscape}
